ViSeRet: A simple yet effective approach to moment retrieval via fine-grained video segmentation

Video-text retrieval has many real-world applications such as media analytics, surveillance, and robotics. This paper presents the 1st place solution to the video retrieval track of the ICCV VALUE Challenge 2021. We present a simple yet effective approach to jointly tackle two video-text retrieval tasks (video retrieval and video corpus moment retrieval) by leveraging the model trained only on the video retrieval task. In addition, we create an ensemble model that achieves the new state-of-the-art performance on all four datasets (TVr, How2r, YouCook2r, and VATEXr) presented in the VALUE Challenge.

==> two-stage.tex <==
Our approach is greatly inspired by the two-stage framework (retriever and reader) that is widely adopted in the NLP open-domain question answering(ODQA) tasks: the retriever model first selects a small number of passage candidates from a large pool of text corpus. Then, the reader model processes each passage candidate to find more precise answer(span) within the passage and re-rank the items based on the new score.

Our approach brings this two-stage framework to the text-to-video tasks: (1) video \textit{retriever} model: we segment each video into several fixed-length (i.e., 5 seconds, 10 seconds) clips(i.e., passage), treating them as separate videos, and select a small number of candidate video clips (2) video \textit{reader} model: we fine-grain the start and end time of each segmented video clip and re-rank them based on the weighted sum of the retriever model and the reader model scores. For the video retrieval task, we ignore the reader model and only use the retrieval model's results without any slicing process. 
Our overall methodology is greatly inspired by the two-stage framework (retriever and reader) that is widely adopted in the NLP open-domain question answering(ODQA) tasks: the retriever model first selects a small number of passage candidates from a large pool of text corpus. Then, the reader model processes each passage candidate to find more precise answer(span) within the passage and re-rank the items based on the new score.

The main ground for this approach is to utilize the performance of the retrieval model[MMT, CLIP4CLIP] to its maximum and have the reader fine-grain the retrieval model's results.


%-------------------------------------------------------------------------
\subsection{Stage 2: Video Reader Model}

Video reader model aims to locate the relevant moment in the retrieved video clip. Temporal moment localization candidates per query-video clip are ranked by summation of start and end scores by video reader model. Final Video Corpus Moment Retrieval(VCMR) scores are re-ranked by summation of weighted scores of video retrieval model and video reader model. 
We investigate retriever only model can replace reader model by segmenting origin video clip into several segment units and using segment information as start and end time span. Because TVR and How2R data sets have various queries with different characteristics within same video clips, representing all video clips in the same space can degrade performance of video retriever model. Video reader model can be used to fine-grain the start and end times of a segmented video clips.

We also experiment the impact of input channels using different video reader model for subtitle only and visual-subtitle input. For subtitle only input, we use transformer based model, and for visual-subtitle input same model as retriever is used.

\subsubsection{Subtitle only Reader model}
\textbf{Model Architecture} 
To investigate the possibility of replacing a video reader with video retriever model with segmented video clips, we reconstruct the subtitle data to only use segmented video clips which is identical to the video retriever setup. Without segment video clip setting, we use all subtitle information to find relevant moment for query as a video reader input.

Subtitle only video reader model uses Transformer based encoder and two fully connected layer. Especially it uses DistillBERT model which is lighter and faster than BERT. Query and according subtitle pairs are used as an input separated by SEP token. Two linear layers on top of output embedding are used to predict start and end indexes respectively. Each token index is mapped to timestamp information using linear interpolation, so moment localization task becomes a classification problem. In VCMR task, weighted sum of retriever score and reader score is used.

\textbf{Training} We compared two types of inputs in video reader model training. First one is using all context as input, and second one is using sliced context which is using subtitle information only within segment timestamp. We find sliced context setting performs better than all context setting in moment localization, so we focus on the segmented context in this experiment. The model is trained from scratch and the best performing model on the validation set with a meta average recall score of 1,5,10 is chosen.

\textbf{Inference} Model receives query-clip context candidates as inputs, and predicts start and end index separately. The sum of the starting and ending logits with the starting index less than the ending index is used as the reader score. Final scores are re-ranked by weighted summation of video retriever score and each span's score. 
When re-rank scores are above threshold, which can be interpreted as video reader model is reliable, we use reader predicted time span as model outputs. Otherwise we use time segment information of segmented video clips as the model output instead.

\subsubsection{Subtitle + Video Reader model}
\textbf{Model Architecture} Subtitle + Video reader model uses same architecture as video retriever model to get video and query embedding. Query-video similarity score is calculated between the query and the video embedding using dot product. And we use two convolution filters on top of the scores, followed by a softmax layer to predict start and end index following XML setting [XML].

(Q.How to mention subtitle + video reader model when we couldn't complete the experiments?)
%-------------------------------------------------------------------------



\textbf{Subtitle only Video Reader Model} Video reader model is trained with cross entropy loss. We used DistillBERT for query-subtitle pair encoding. The batch size is 128 with learning rate 5e-5. The model is optimized by AdamW. 
For the How2R data set, the thresholds for the start and end logits are set to 6.0, which is determined by the validation distribution. When video reader model's logit is under the threshold, we use time segmented information of retriever input. We find that for TVR data set model output is unstable, so it is hard to find proper threshold. In this case, we just use segmented timestamp information of segmented video clips for model predicted timestamp. 
In our experiment we find that by only using retriever model we can replace reader module and outperforms the baseline. And the usage of extra reader module doesn't give meaningful performance gain, so we simply focus on retriever model to perform VCMR task alone by using the segmented timestamp information. 

